300 GHz Wideband Channel Measurement and Analysis in a Lobby

The Terahertz (0.1-10 THz) band has been envisioned as one of the promising spectrum bands to support ultra-broadband sixth-generation (6G) and beyond communications. In this paper, a wideband channel measurement campaign in a 500- square-meter indoor lobby at 306-321 GHz is presented. The measurement system consists of a vector network analyzer (VNA)-based channel sounder, and a directional antenna equipped at the receiver to resolve multi-path components (MPCs) in the angular domain. In particular, 21 positions and 3780 channel impulse responses (CIRs) are measured in the lobby, including the line-of-sight (LoS), non-line-of-sight (NLoS) and obstructed-line-of-sight (OLoS) cases. The multi-path characteristics are summarized as follows. First, the main scatterers in the lobby include the glass, the pillar, and the LED screen. Second, best direction and omni-directional path losses are analyzed. Compared with the close-in path loss model, the optimal path loss offset in the alpha-beta path loss model exceeds 86 dB in the LoS case, and accordingly, the exponent decreases to 1.57 and below. Third, more than 10 clusters are observed in OLoS and NLoS cases, compared to 2.17 clusters on average in the LoS case. Fourth, the average power dispersion of MPCs is smaller in both temporal and angular domains in the LoS case, compared with the NLoS and OLoS counterparts. Finally, in contrast to hallway scenarios measured in previous works at the same frequency band, the lobby which is larger in dimension and square in shape, features larger path losses and smaller delay and angular spreads.

==> contents/hallway_ref/CAMPAIGN_hallway.tex <==
\section{Channel Measurement Campaign} \label{section: campaign}

In this section, we describe the 306-321~GHz measurement campaign as well as the data post-processing procedures in the L-shaped hallway. The measurement is carried out on the second floor of the Longbin building, at the University of Michigan-Shanghai Jiao Tong University Joint Institute (UM-SJTU JI), Shanghai Jiao Tong University (SJTU).
% First, we introduce the specification of the hardware system, the environment of the test scene, and the measurement deployment. Second, system calibration is carried out to eliminate the impact of the measurement system on the channel. Third, MPC extraction and clustering is implemented to post-process the received multi-path signals.

\subsection{Channel Measurement System}
We adopt a 260-400~GHz channel measurement platform that consists of radio frequency (RF) fronts supported by a Ceyear 3672C VNA. The VNA supports the frequency range from 10~MHz to 43.5~GHz. Standard waveguides WR2.8 are integrated with both Tx and Rx modules, while a horn antenna is installed at the Rx side. The Tx waveguide has a gain of around 7~dBi, while the Rx antenna has a half-power beamwidth (HPBW) of $8^\circ$ and an antenna gain around 25-27~dBi at 260-400~GHz.
In this measurement campaign, the frequency band of 306-321~GHz is investigated. The measured bandwidths is 15~GHz, which denotes that the time and space resolutions are 66.7~ps and 2~cm, respectively. The frequency sweeping interval is 2.5~MHz, resulting in 6001 sweeping points and a maximum excess delay of 400~ns, which is equivalent to a maximum detectable path length of 120~m. The noise floor of the THz measurement platform is -180~dBm, and the dynamic range is 119~dB.

As shown in Fig.~\ref{fig:platform}, the transceiver module is mounted on a rotator. The Tx is placed on an electric lifter, which is integrated with the electric cart, to reach the height of 2~m above the ground. By contrast, the Rx is put on the top of the cart without a lifter, which results in the height of 1.75~m above the ground. The Tx is static at zero azimuth and elevation angles. Motored by the rotator, the Rx scans from $0^\circ$ to $360^\circ$ in the azimuth domain and from $-20^\circ$ to $20^\circ$ in the elevation domain to receive multi-path propagation, with the angle step of $10^\circ$. Key parameters of the measurement system are summarized in Table~\ref{tab:system_parameter}.
% As shown in Fig.~\ref{fig:platform}, Tx and Rx modules are mounted on rotators. The Tx is static at zero azimuth and elevation angles, while the Rx scans, with the angle resolution of $10^\circ$, from $0^\circ$ to $360^\circ$ in the azimuth domain and $-20^\circ$ to $20^\circ$ in the elevation domain to receive multi-path propagation. The combination of rotator and Tx is placed on an electric lifter, which is integrated with the electric cart, to reach the height of 2~m above the ground. By contrast, the combination of rotator and Rx is directly put on the top of the cart, with the height of 1.75~m above the ground. Key parameters of the measurement system are summarized in Table~\ref{tab:system_parameter}.

\begin{figure}
    \centering
    %\subfigure[The transmitter side.]{
    \includegraphics[width=0.75\linewidth]{figures/platform_tx_front.png}
    %}
    %\subfigure[The receiver side.]{
    %\includegraphics[width=0.45\linewidth]{figures/platform_rx.png}
    %}
    \caption{Channel measurement system.}
    \label{fig:platform}
\end{figure}

\begin{table}[htbp]
  \centering
  \caption{Parameters of the measurement system.}
    \begin{tabular}{ll}
    \toprule
    Parameter & Value \\
    \midrule
    Frequency band              & 306-321~GHz \\
    Bandwidth                   & 15~GHz \\
    Sweeping interval           & 2.5~MHz \\
    Sweeping points             & 6001 \\
    Tx antenna gain & 7~dBi \\
    Rx antenna gain  & 25-27~dBi \\
    HPBW of Rx antenna          & $8^\circ$ \\
    Time resolution             & 66.7~ps \\
    Space resolution            & 2~cm \\
    Maximum excess delay        & 400~ns \\
    Maximum path length         & 120~m \\
    Rx azimuth rotation range   & $[0^\circ:10^\circ:360^\circ]$ \\
    Rx elevation rotation range & $[-20^\circ:10^\circ:20^\circ]$ \\
    Average noise floor         & -180~dBm \\
    Dynamic range               & 119~dB \\
    \bottomrule
    \end{tabular}
  \label{tab:system_parameter}
\end{table}


\subsection{Measurement Deployment}
The measurement campaign is conducted in the L-shaped hallway on the second floor of the building of UM-SJTU JI. As shown in Fig.~\ref{fig:deployment}(a), the campaign mainly consists of two perpendicular corridors, connected by a corner. The long corridor is 2.97~m wide and 32.53~m long (between Wall~A and Wall~B), including two 3~m long extensions at both ends. Indented offices are distributed along the corridor, whose depth is about 0.6~m with doors closed. The other corridor is 7~m wide (between Wall~C and Wall~D) which extends all the way to the left end. The measurement deployment is illustrated in Fig.~\ref{fig:deployment}(b). Tx is placed in the long corridor, together with four LoS Rx positions, while nine NLoS Rx positions are located in the wide corridor. Since signals are too weak to be detected in the wide corridor far from the corner, the rest of the wide corridor to the left end is omitted in Fig.~\ref{fig:deployment}(b).

\begin{figure}
    \centering
    \subfigure[The photo of the measurement campaign.]{
    \includegraphics[width=0.76\linewidth]{figures/deployment_photo.png}
    }
    \\
    \subfigure[Measurement deployment (unit: mm).]{
    \includegraphics[width=0.95\linewidth]{figures/deployment_13pts.png}
    }
    \caption{Measurement campaign and deployment in an L-shaped hallway, 2$^{\rm nd}$ floor of UM-SJTU JI building, SJTU.}
    \label{fig:deployment}
\end{figure}


\begin{comment}

\subsection{System Calibration}
%\begin{figure}
%    \centering
%    \subfigure[Measurement.]{
%    \includegraphics[width=0.6\linewidth]{figures/measure_structure.png}
%    }
%    \subfigure[Calibration.]{
%    \includegraphics[width=0.55\linewidth]{figures/calibration_structure.png}
%    }
%    \caption{The system structure in the (a) measurement, and (b) calibration.}
%    \label{fig:calib}
%\end{figure}

Before data processing, system calibration is carried out to eliminate the effect of the measurement system, namely, the VNA, RF fronts, and cables. In other words, the measured S21 parameter from the measurement system, $S_{\rm measure}$ is expressed as
\begin{equation}
    S_{\rm measure} = H_{\rm system} H_{\rm channel} H_{\rm Tx,waveguide} H_{\rm Rx,antenna},
\end{equation}
where $H_{\rm system}$ is the response of the sounder and $H_{\rm channel}$ denotes the transfer function of the realistic wireless channel that signals went through in the scenario. $H_{\rm Tx,waveguide}$ and $H_{\rm Rx,antenna}$ represent the directivity of the waveguide at Tx and the antenna at Rx, respectively.
To take out $H_{\rm system}$, 
%as shown in Fig.~\ref{fig:calib}(b),
we removed the Rx antenna and directly concatenated two RF fronts, with the addition of a 40-dB attenuator to protect the device. Therefore, the S21 parameter given by the calibration, $S_{\rm calib}$, is composed of
\begin{equation}
    S_{\rm calib} = H_{\rm system} H_{\rm attenuator},
\end{equation}
where $H_{\rm attenuator}$ is the response of the attenuator.
Combination of the two equations yields
\begin{equation}
    H_{\rm channel} = \frac{S_{\rm measure}} {S_{\rm calib}} \times \frac{H_{\rm attenuator}}{H_{\rm Tx,waveguide} H_{\rm Rx,antenna}},
\end{equation}
where $H_{\rm Tx,waveguide}$ (7~dBi), $H_{\rm Rx,antenna}$ (25-27~dBi) and $H_{\rm attenuator}$ (-40~dB) are already known.
% Since the waveguide is integrated with the RF front, we further implemented an experiment to calculate the Tx waveguide directivity $H_{\rm Tx,waveguide}$. In the experiment, we aligned the Tx and Rx within a short distance and measured S21 parameters twice. In the first time, the system structure is the same as Fig.~\ref{fig:calib}(a), while in the other, an identical antenna is added to the front of the Tx. Hence, the difference between the two measured S21 is equal to the directivity difference between the Tx waveguide and the antenna. By subtraction of the S21 difference from the known antenna directivity, the result of the Tx waveguide directivity is about 7~dBi at 306-321~GHz.
% derived as shown in Fig.~\ref{fig:waveguide_gain}.
%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{figures/waveguide_gain.png}
%    \caption{Directivity of the waveguide at the Tx.}
%    \label{fig:waveguide_gain}
%\end{figure}

\end{comment}

\subsection{MPC Extraction and Clustering}
Before data processing, system calibration is carried out to eliminate the effect of the measurement system~\cite{he2021channel}.
% MPC Extraction
For each Tx-Rx direction pair, we obtain 6001 samples of channel impulse response (CIR) $h_{\rm channel}$ from the inverse discrete Fourier transform (IDFT) of the channel transfer function (CTF) $H_{\rm channel}$. Instead of applying the Space-Alternating Generalized Expectation-maximization (SAGE) algorithm, we regard each sample as one possible MPC in the temporal domain, for the following two reasons. First, the high-resolution SAGE algorithm is susceptible to phase inaccuracy caused by cable swing during the rotation of the Rx. Second, SAGE requires accurate 3D antenna pattern, which is not available in our case~\cite{wu201760}.
% Noise Elimination
Therefore, we extract MPCs from CIR samples after noise samples are eliminated. Noise samples refer to those with power lower than the threshold, which is given by
\begin{equation}
    P_{\rm TH} \text{ [dB]} = \max\{P_{\rm m}-40, \text{NF}+10\},
\end{equation}
where $P_{\rm m}$ denotes the maximum power among measured samples, and NF is the average noise floor.
After noise elimination, the azimuth and elevation angles of the Rx are considered as the azimuth and elevation angles-of-arrival (AoAs) of each MPC, respectively. The delay of receiving the sample is equal to the time-of-arrival (ToA) of the corresponding MPC.

% Clustering
Furthermore, MPCs are grouped into clusters based on the Density-Based Spatial Clustering of Applications with Noise (DBSCAN) algorithm. Since a cluster typically contains one primary reflected path and surrounding scattered paths, multi-path component distance (MCD) is adapted in the DBSCAN algorithm, which allows MPCs with similar ToA and AoA to be grouped into a cluster~\cite{chen2021channel}. In particular, MCD is defined as
\begin{equation}
    MCD = \sqrt{ d^2 + \xi{d_{\tau}}^2 },
\end{equation}
where $\xi$ indicates the weight of temporal difference, and equals to 4 in this work. $d$ and $d_{\tau}$ represent the distances between two MPCs in the spatial and temporal domains, respectively, described as
\begin{subequations}
    \begin{equation}
    d = \left\| \begin{pmatrix}
        \cos(\theta_{i})\cdot\cos(\varphi_{i}) - \cos(\theta_{j})\cdot\cos(\varphi_{j})\\
        \cos(\theta_{i})\cdot\sin(\varphi_{i}) - \cos(\theta_{j})\cdot\sin(\varphi_{j})\\
        \sin(\theta_{i})-\sin(\theta_{j})
        \end{pmatrix} \right\|_2,
    \end{equation}
    \begin{equation}
    d_{\tau} = | \tau_{i} - \tau_{j} |/\tau_{\rm m},
    \end{equation}
\end{subequations}
where $\theta_{i/j}$ and $\varphi_{i/j}$ represent the elevation and azimuth AoA the $i/j$-th MPC, $\tau_{i/j}$ is the ToA of the $i/j$-th MPC, and $\tau_{\rm m}$ denotes the maximum ToA among all MPCs.

==> contents/hallway_ref/RESULTS_hallway.tex <==
\section{Channel Analysis and Characterization} \label{section: results}
In this section, multi-path propagation and clustering analysis in the measured L-shaped hallway are presented. Moreover, channel characteristics are analyzed in depth, including path loss, delay spread, angular spread, and temporal arrival of clusters.

\subsection{Multi-path Propagation and Clustering Analysis} \label{sec:MPC_analysis} 

\subsubsection{LoS case} \label{sec:MPC_analysis_LoS} % cluster
We first take Rx1 in the LoS case as an example, and analyze the spatial and temporal distributions of MPCs in the LoS indoor hallway scenario.
As shown in Fig.~\ref{fig:clustering_pt1}, cluster~1 denotes the cluster consisting of the LoS ray and some scattering paths, with the largest cluster power and the ToA of 26~ns, i.e., the travelling distance of 7.8~m.
Cluster~2, 3, and 4 are reflected from the indented offices distributed along the corridor. As shown in Fig.~\ref{fig:clustering_pt1}(a) and (b), the values of the azimuth AoA and the ToA are in well accordance with the office locations in the campaign.
Besides, cluster~5 results from the reflections between the two electric carts of Tx and Rx. This is verified by the value of ToA 77~ns, which is about three times the ToA of the LoS cluster, i.e., the MPCs are reflected by the carts twice and travel three times the distance between the Tx and the Rx, as shown in Fig.~\ref{fig:clustering_pt1}(b).
Cluster~6 represents the first-order reflection by one end of the long corridor, for which the ToA of 144~ns indicates the traveling distance of 43.2~m.
By contrast, Cluster~7, which immediately follows Cluster~6, travels 48~m, and possibly refers to the reflected rays by the floor and the ceiling.
Furthermore, Cluster~8 is the second-order reflection by two ends of the long corridor. The ToA of 246~ns indicates the traveling distance of 73.8~m, which is larger than that of the LoS cluster by 56~m, about twice the length of the long corridor.
% Note that there exists a cluster with azimuth AoA of $180^\circ$, ToA of 30~ns, and contains MPCs only with negative elevation AoAs, which is the reflection from the electric lifter, and is manually deleted in the clustering result.
\begin{figure}
    \centering
    %\subfigure[Measured PDAP at Rx1.]{
    %\includegraphics[width=0.9\linewidth]{figures/PDAP_sc3pt1_306-321.png}
    %}
    %\\
    \subfigure[Clustering result at Rx1.]{
    \includegraphics[width=0.95\linewidth]{figures/cluster_7_0.18_6_sc3pt1_306-321_del.png}
    }
    \\
    \subfigure[Multi-path analysis at Rx1 (unit: mm).]{
    \includegraphics[width=0.95\linewidth]{figures/pt1_MPC_analysis_2_del.png}
    }
    \caption{Clustering result and multi-path analysis at Rx1.}
    \label{fig:clustering_pt1}
\end{figure}

\subsubsection{NLoS case} % MPC PDAP
We take Rx5 to Rx7 in the NLoS case as examples and analyze the spatial and temporal distributions of MPCs in the NLoS indoor hallway scenario. The PDAP results are shown in Fig.~\ref{fig:pdap_pt567}.
First, MPCs mainly come from the corner and travel at least 22.5~m to reach the NLoS points. Besides, NLoS MPCs traveling a long distance (more than 60~m in our case) are too weak to be detected. Therefore, the majority of MPCs are concentrated in the azimuth AoA ranging from 0 to 180$^\circ$ and the ToA ranging from 75 to 200~ns, where we mainly explore the trend of MPCs. Second, as the Rx position farther away from the corner (i.e., from Rx5 to Rx7), intuitively, MPCs travel a longer distance and thus have larger ToAs. At the same time, azimuth AoAs tend to converge towards $\varphi=90^\circ$ (the white dotted lines in Fig.~\ref{fig:pdap_pt567}), which is the direction pointing perpendicular to the long corridor. The observation gives a clue for the existence of certain fixed scattering points on Wall~C and Wall~D adjacent to the corner.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/pdap_pt5-7.png}
    \caption{Measured PDAP at Rx5, Rx6, and Rx7.}
    \label{fig:pdap_pt567}
\end{figure}

\subsubsection{Number of clusters}
According to the MCD-based DBSCAN algorithm, the number of clusters at each Rx position is summarized in Table~\ref{tab:parameters}. The number of cluster does not vary drastically in the LoS case. Besides, when the NLoS Rx position is near the corner (e.g. Rx5, Rx8, and Rx11-13), due to the abundant scattering, the cluster number is comparable to or even larger than that in the LoS case, despite the lack of LoS and reflected clusters. By contrast, when the NLoS Rx positions move farther, e.g. from Rx5 to Rx7 and from Rx8 to Rx10, the cluster number decreases due to the larger path loss.



\subsection{Characteristic Analysis}
% Next, we analyze THz indoor channel characteristics, including path loss, delay spread, angular spread, and temporal arrival of clusters.

\subsubsection{Path loss}
% Large-scale fading is investigated by analyzing the best direction and omni-directional path losses of the LoS path. A close-in free space reference distance (CI) path loss model is invoked based on the measurement results in Sec.~\ref{sec:MPC_analysis}.

The path loss is divided into best direction path loss and omni-directional path losses. For each pair of Tx and Rx positions, the best direction path loss is defined as the loss of the MPC from the best direction which has the strongest received power. By contrast, the omni-directional path loss sums the received power from all directions. The two path losses are respectively given by
\begin{subequations}
    \begin{equation}
    \text{PL}_{\rm best} \text{ [dB]} = -10\cdot\log_{10} \left( \max_{i,j}\{P_{i,j}\} \right),
    \end{equation}
    \begin{equation}
    \text{PL}_{\rm omni} \text{ [dB]} = -10\cdot\log_{10} \left( \sum_{i,j}P_{i,j} \right),
    \end{equation}
\end{subequations}
where $P_{i,j}$ denotes the received power from the $i^{\rm th}$ azimuth angle and the $j^{\rm th}$ elevation angle, as
\begin{equation}\label{eq:power_sum}
    P_{i,j} = \sum_{t}|h_{i,j,t}|^2,
\end{equation}
where $h_{i,j,t}$ represents the CIR at the $t^{\rm th}$ sample time point from, the $i^{\rm th}$ azimuth and the $j^{\rm th}$ elevation angles.

The close-in free space reference distance (CI) model is invoked based on the results of best direction and omni-directional path losses, respectively. The CI path loss model is expressed as
\begin{equation}
    \text{PL}^{\rm CI} = 10\times\text{PLE}\times\log_{10}\frac{d}{d_0}+\text{FSPL}(d_0)+X_{\sigma_{\rm SF}},
\end{equation}
where PLE is the path loss exponent, $d$ denotes the distance between Tx and Rx, and $d_0$, which is 1~m in this work, represents the reference distance. $X_{\sigma_{\rm SF}}$ is a zero-mean Gaussian random variable with standard deviation $\sigma_{\rm SF}$ in dB, indicating the fluctuation caused by shadow fading. Furthermore, the free-space path loss (FSPL) is given by the Friis’ law, as
\begin{equation}
    \text{FSPL}(d,f) = -20\times\log_{10}\frac{c}{4\pi f d},
\end{equation}
where $f$ denotes the frequency, and $c$ is the speed of light.
We determine the values of PLE in the CI model by minimizing $\sigma_{\rm SF}$. The fitting results are shown in Fig.~\ref{fig:pl}. The measurement results yield that the PLE value is 1.7222 for the best direction path loss and 1.3910 for the omni-direction path loss, respectively.
Justifications are elaborated as follows.
First, due to the waveguide effect, besides the LoS ray, strong reflected paths with different ToAs can also be detected from the best direction. Thus, the received power is increased by the summation of received power in the \textit{time} domain, as expressed in~\eqref{eq:power_sum}. As a result, the best direction path loss is reduced, and the PLE value is smaller than 2, which is the PLE for ideal free-space path loss.
Second, the omni-directional received power sums the received power in both \textit{time} and \textit{angular} domains. To be specific, besides paths from the best direction, reflected paths from the south, and scattered paths from all other directions are included in the summation of~\eqref{eq:power_sum}, resulting in a smaller PLE for the omni-directional path loss.
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/path_loss_sc3_los_306-321_(fix G_Tx=7).png}
    \caption{Path loss measurement and fitted CI models.}
    \label{fig:pl}
\end{figure}


\subsubsection{Delay and angular spreads}
We use the root-mean-square (RMS) delay spread (DS) and azimuth spread of angle (ASA) to measure the power dispersion of MPCs in temporal and spatial domains, respectively.
%\begin{subequations}
%    \begin{equation}
%        \tau_{\rm RMS} =  \sqrt{\frac{\sum_{i=1}^{N}(\tau_i-\bar{\tau})^2P_i}{\sum_{i=1}^{N}P_i}},
%    \end{equation}
%    \begin{equation}
%        \varphi_{\rm RMS} = \min_{\Delta\varphi\in[0,\varphi_{\rm m}]} \sqrt{\frac{\sum_{i=1}^{N}(\varphi_i+\Delta\varphi-\bar{\varphi})^2P_i}{\sum_{i=1}^{N}P_i}},
%    \end{equation}
%\end{subequations}
%and
%\begin{subequations}
%    \begin{equation}
%        \bar{\tau} = \frac{\sum_{i=1}^{N}\tau_iP_i}{\sum_{i=1}^{N}P_i},
%    \end{equation}
%    \begin{equation}
%        \bar{\varphi} = \frac{\sum_{i=1}^{N}(\varphi_i+\Delta\varphi)P_i}{\sum_{i=1}^{N}P_i},
%    \end{equation}
%\end{subequations}
%where $N$ is the number of MPCs, $\tau_i$, $\varphi_i$, and $P_i$ denote the ToA, the azimuth AoA, and the power of the $i^{\rm th}$ MPC. $\tau_{\rm m}$ represents the maximum excess delay, which is 400~ns in this work, and $\tau_{\rm m}$ is 360$^\circ$.
%where $N$ is the number of MPCs, $\tau_i$ and $P_i$ denote the ToA and the power of the $i^{\rm th}$ MPC. $\tau_{\rm m}$ represents the maximum excess delay, which is 400~ns in this work. The RMS ASA can be derived in a similar way. Detailed results are summarized in Table~\ref{tab:parameters}.
In the LoS case, the values of DS are around 20~ns, except for Rx1 due to the reflection from offices, as illustrated in Fig.~\ref{fig:clustering_pt1}. The value of ASA increases as the position of Rx moves closer to the corner. 
% This is explained by Fig.~\ref{fig:clustering_pt4}, where many MPCs, though do not form any cluster, are detected as reflected and scattered rays from the corner at the azimuth AoA around 180$^\circ$.
This is caused by MPCs which are reflected and scattered between the corner and the cart. These MPCs arrive at the Rx with the azimuth AoA around 180$^\circ$. As a result, the increase of received power from the south (with $\varphi$ near $180^\circ$) counterweights the power of MPCs from the north (with $\varphi$ near $0^\circ$ or $360^\circ$), and results in a larger ASA.
%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{figures/cluster_7_0.18_6_sc3pt4_306-321.png}
%    \caption{Clustering result at Rx4.}
%    \label{fig:clustering_pt4}
%\end{figure}

In the NLoS case, since MPC power is comparable to the noise floor, values of DS and ASA are highly dependent on the dominated MPCs that are scattered by Wall~C and Wall~D adjacent to the corner. When Rx moves farther away from the corner, some of these MPCs become weaker and are overwhelmed under the noise level, which renders inconclusive changes of DS and ASA. Though, in the general sense, the average DS and ASA of the NLoS case are 28~ns and 47$^\circ$, which are still larger than the counterparts in the LoS case, i.e., 18~ns and 33$^\circ$.



\subsubsection{Temporal arrival of clusters}
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/cluster_delay_diff_13pts.png}
    \caption{Distribution of cluster delay difference.}
    \label{fig:cluster_delay_diff}
\end{figure}
Furthermore, the temporal arrival of the clusters is often modeled by a Poisson process~\cite{ju2021millimeter}, which indicates that the delay difference $\Delta\tau$ between two successive clusters is exponentially distributed. Based on the clustering result, the distribution of cluster delay difference $\Delta\tau$ shows a good agreement with the exponential fitting, as portrayed in Fig.~\ref{fig:cluster_delay_diff}. The average values of the exponential distribution in the LoS and NLoS case are 37.15~ns and 22.59~ns, respectively.
Specifically, the NLoS case mainly observes scattering clusters that travel between Wall~C and Wall~D, and the path length difference is about the width of the wide corridor, 7.2~m. In the LoS case, by contrast, LoS and wall-reflected clusters dominate, which travel between Wall~A and Wall~B. Thus, the path length difference is about the length of the long corridor, 32.53~m. Besides, between the LoS and wall-reflected clusters, as discussed in Sec.~\ref{sec:MPC_analysis_LoS}, we recognize additional clusters from the carts and the offices. The existence of these in-between clusters decreases the inter-cluster delay difference $\Delta\tau$. Despite this, the average value of cluster delay difference in the LoS case is still larger than that in the NLoS case.
% Specifically, the NLoS case mainly observes scattering clusters, whose traveling distance gaps approximate the width of the wide corridor. By contrast, in the LoS case, LoS and wall-reflected clusters dominate, whose traveling distance gaps approximate the length of the long corridor. In between, the cart and the office produce additional clusters which decrease the delay difference. Despite this, the average value of cluster delay difference in the LoS case is still larger than that in the NLoS case.



%\subsubsection{Intra-cluster delay spread}
%\subsubsection{Intra-cluster angular spread}
%\subsubsection{Cluster power versus excess delay}




%\subsection{Comparison between two bands (?)}


\begin{table*}
\caption{Summary of channel parameters in the L-shaped indoor hallway at 306-321~GHz.}
\label{tab:parameters}
\centering
%\resizebox{\linewidth}{!}{
%\begin{tabular}{@{}c|cccc|cccccc@{}}
%\toprule
%\multirow{2}{*}{Point index} & \multicolumn{4}{c|}{LoS} & \multicolumn{6}{c}{NLoS} \\ \cmidrule(l){2-11} & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
%\midrule
%DS [ns] & 10.19 & 21.58 & 19.26 & 20.69 & 20.91 & 61.57 & 29.06 & 33.09 & 22.15 & 25.84 \\
%ASA [$^\circ$] & 19.96 & 29.04 & 31.52 & 52.10 & 38.92 & 70.67 & 36.23 & 48.99 & 56.29 & 24.28 \\
%Cluster number & 8 & 6 & 8 & 6 & 8 & 3 & 0 & 9 & 3 & 2  \\
%\bottomrule
%\end{tabular}
%}
\includegraphics[width=0.92\linewidth]{figures/parameters_13pts.png}
\end{table*}
